PSALTer: Particle Spectrum for Any Tensor Lagrangian

We present the PSALTer software for efficiently computing the mass and energy of the particle spectrum for any (e.g. higher-rank) tensor field theory in the Wolfram Language. The user must provide a Lagrangian density which is expanded quadratically in the fields around a Minkowski vacuum, is linear in the coupling coefficients, and otherwise built from the partial derivative and Minkowski metric. PSALTer automatically computes the spin-projection operators, saturated propagator, bare masses, residues of massive and massless poles and overall unitarity conditions in terms of the coupling coefficients. The constraints on the source currents and total number of gauge symmetries are produced as a by-product. We provide examples from scalar, vector, tensor and gauge theories of gravity. Each example, including spectra of higher-spin modified gravity theories, may be obtained on a personal computer in a matter of minutes. The software is also parallelised for use on high-performance computing resources. The initial release allows for parity-preserving operators constructed from fields of up to rank three: this functionality will be extended in future versions. PSALTer is a contribution to the xAct project.

==> LstListing/Line1.tex <==
In[#]:= Print["Hello world."]; 

==> LstListing/Line10.tex <==
In[#]:= Print[Information["$ReadOnly", LongForm -> False]]; $ReadOnly = False; 

==> LstListing/Line100.tex <==
In[100]:= ParticleSpectrum[-1/3 * (kT1 * SpinConnection[-i, a, i] * SpinConnection[-k, -a, k]) - kT1 * SpinConnection[-i, k, l] * SpinConnection[-k, -l, i] + kR1 * CD[-i][SpinConnection[k, l, -k]] * CD[i][SpinConnection[-l, a, -a]] - (2 * kR1 * CD[b][SpinConnection[j, a, -k]] * CD[-j][SpinConnection[-a, -b, (*omitted 2274 characters for brevity*) a, -j]] * CD[l][SpinConnection[j, k, -k]] - 3 * kR1 * CD[-j][SpinConnection[-l, a, -a]] * CD[l][SpinConnection[j, k, -k]] + 4 * kR3 * CD[-j][SpinConnection[-l, a, -a]] * CD[l][SpinConnection[j, k, -k]], TheoryName -> StringJoin["Case", ToString[58]], Method -> "Easy", MaxLaurentDepth -> 3];

==> LstListing/Line101.tex <==
In[101]:= DefField[Connection[-a, -b, -c], PrintAs -> "\[CapitalGamma]", PrintSourceAs -> "\[CapitalDelta]"]; 

==> LstListing/Line102.tex <==
In[102]:= DefConstantSymbol[A0, PrintAs -> "\!\(\ * SubscriptBox[\(\[ScriptA]\), \(0\)]\)"]; DefConstantSymbol[A1, PrintAs -> "\!\(\ * SubscriptBox[\(\[ScriptA]\), \(1\)]\)"]; DefConstantSymbol[A2, PrintAs -> "\!\(\ * SubscriptBox[\(\[ScriptA]\), \(2\)]\)"]; DefConstantSymbol[A3, PrintAs -> "\!\(\ * SubscriptBox[\(\[ScriptA]\), \(3\)]\)"]; (*omitted 1490 characters for brevity*) PrintAs -> "\!\(\ * SubscriptBox[\(\[ScriptC]\), \(13\)]\)"]; DefConstantSymbol[C14, PrintAs -> "\!\(\ * SubscriptBox[\(\[ScriptC]\), \(14\)]\)"]; DefConstantSymbol[C15, PrintAs -> "\!\(\ * SubscriptBox[\(\[ScriptC]\), \(15\)]\)"]; DefConstantSymbol[C16, PrintAs -> "\!\(\ * SubscriptBox[\(\[ScriptC]\), \(16\)]\)"];

==> LstListing/Line103.tex <==
In[103]:= ParticleSpectrum[-1/2 * (A0 * Connection[a, b, c] * Connection[-b, -c, -a]) + (A0 * Connection[a, -a, b] * Connection[c, -b, -c])/2 - (A0 * MetricPerturbation[c, -c] * CD[-b][Connection[a, -a, b]])/4 + (A0 * MetricPerturbation[c, -c] * CD[-b][Connection[a, b, -a]])/4 - (A0 * MetricPerturbation[-a, -c] * CD[-b][Connection[a, b, c]])/2 + (A0 * MetricPerturbation[-b, -c] * CD[c][Connection[a, -a, b]])/2, TheoryName -> "MetricAffineEinsteinHilbertTheory", Method -> "Hard", MaxLaurentDepth -> 3]; 

==> LstListing/Line104.tex <==
In[104]:= ParticleSpectrum[-1/2 * (A0 * Connection[a, b, c] * Connection[-b, -c, -a]) + (A0 * Connection[a, -a, b] * Connection[c, -b, -c])/2 - (A0 * MetricPerturbation[c, -c] * CD[-b][Connection[a, -a, b]])/4 + (A0 * MetricPerturbation[c, -c] * CD[-b][Connection[a, b, -a]])/4 - (A0 * MetricPerturbation[-a, -c] * CD[-b][Connection[a, b, c]])/2 - (A0 * Connection[a, b, c] * CD[-b][MetricPerturbation[-a, -c]])/2 - (A0 * Connection[a, -a, b] * CD[-b][MetricPerturbation[c, -c]])/4 + (A0 * Connection[a, b, -a] * CD[-b][MetricPerturbation[c, -c]])/4 + (A0 * MetricPerturbation[a, b] * CD[-b][CD[-a][MetricPerturbation[c, -c]]])/2 - (A0 * CD[-b][MetricPerturbation[c, -c]] * CD[b][MetricPerturbation[a, -a]])/8 + (A0 * Connection[a, -a, b] * CD[-c][MetricPerturbation[-b, c]])/2 - (A0 * CD[-a][MetricPerturbation[a, b]] * CD[-c][MetricPerturbation[-b, c]])/2 + (A0 * CD[b][MetricPerturbation[a, -a]] * CD[-c][MetricPerturbation[-b, c]])/2 - A0 * MetricPerturbation[a, b] * CD[-c][CD[-b][MetricPerturbation[-a, c]]] + (A0 * MetricPerturbation[a, -a] * CD[-c][CD[-b][MetricPerturbation[b, c]]])/4 + (A0 * MetricPerturbation[a, b] * CD[-c][CD[c][MetricPerturbation[-a, -b]]])/2 - (A0 * MetricPerturbation[a, -a] * CD[-c][CD[c][MetricPerturbation[b, -b]]])/4 + (A0 * MetricPerturbation[-b, -c] * CD[c][Connection[a, -a, b]])/2 - (A0 * CD[-b][MetricPerturbation[-a, -c]] * CD[c][MetricPerturbation[a, b]])/4 + (3 * A0 * CD[-c][MetricPerturbation[-a, -b]] * CD[c][MetricPerturbation[a, b]])/8, TheoryName -> "MetricAffineEinsteinHilbertTheorySecondOrder", Method -> "Hard", MaxLaurentDepth -> 3]; 

==> LstListing/Line105.tex <==
In[105]:= ParticleSpectrum[((-2 * A0 + 2 * A1 + A2 - 12 * A6 + 2 * A9) * Connection[-a, m, -m] * Connection[a, b, -b])/6 + ((-A0 + 2 * (-4 * A1 + A5 + 9 * A7 - 2 * A9)) * Connection[-a, -b, -m] * Connection[a, b, m])/8 + ((-A0 + 2 * (-2 * A2 + A5 + 9 * A7 - 2 * A9)) * Connection[-a, -m, -b] * Connection[a, (*omitted 1808 characters for brevity*) n, -n]] * CD[m][Connection[a, b, -b]] - (A0 * CD[-b][MetricPerturbation[-a, -m]] * CD[m][MetricPerturbation[a, b]])/4 + (A0 * CD[-m][MetricPerturbation[-a, -b]] * CD[m][MetricPerturbation[a, b]])/8, TheoryName -> "IsoWeylTheorySecondOrder", Method -> "Hard", MaxLaurentDepth -> 1];

==> LstListing/Line106.tex <==
In[106]:= ParticleSpectrum[((4 * A1 + 2 * A2 + 3 * A3 - 12 * A6 + 2 * A9) * Connection[-a, c, -c] * Connection[a, b, -b])/6 + ((-A0 - 6 * A1 - A2 - 3 * A3 + 8 * A6 + 4 * A7 - 2 * A9) * Connection[-a, -b, -c] * Connection[a, b, c])/4 + ((-A0 - 2 * A1 - 3 * A2 - 3 * A3 + 8 * A6 + 4 * A7 - 2 * A9) * (*omitted 3235 characters for brevity*) b, c]] + C1 * CD[-c][CD[-b][MetricPerturbation[-a, -m]]] * CD[m][CD[c][MetricPerturbation[a, b]]] - C1 * CD[-m][CD[-b][MetricPerturbation[-a, -c]]] * CD[m][CD[c][MetricPerturbation[a, b]]], TheoryName -> "ExtendedProjectiveTheorySecondOrder", Method -> "Hard", MaxLaurentDepth -> 1];

==> LstListing/Line107.tex <==
In[107]:= ParticleSpectrum[-1/2 * (A0 * Connection[a, b, c] * Connection[-b, -c, -a]) + (A0 * Connection[a, -a, b] * Connection[c, -b, -c])/2 - (A0 * MetricPerturbation[c, -c] * CD[-b][Connection[a, -a, b]])/4 + (A0 * MetricPerturbation[c, -c] * CD[-b][Connection[a, b, -a]])/4 - (A0 * MetricPerturbation[-a, (*omitted 3200 characters for brevity*) - (11 * C1 * CD[-b][Connection[-d, -a, b]] * CD[d][Connection[a, c, -c]])/2 - (C1 * CD[a][Connection[-d, -a, b]] * CD[d][Connection[-b, c, -c]])/2 + (C1 * CD[-b][Connection[-d, -a, b]] * CD[d][Connection[c, a, -c]])/2, TheoryName -> "ProjectiveTheory", Method -> "Hard", MaxLaurentDepth -> 1];

==> LstListing/Line108.tex <==
In[108]:= ParticleSpectrum[-1/2 * (A0 * Connection[a, b, c] * Connection[-b, -c, -a]) + (A0 * Connection[a, -a, b] * Connection[c, -b, -c])/2 - (A0 * MetricPerturbation[c, -c] * CD[-b][Connection[a, -a, b]])/4 + (A0 * MetricPerturbation[c, -c] * CD[-b][Connection[a, b, -a]])/4 - (A0 * MetricPerturbation[-a, (*omitted 8137 characters for brevity*) b]]])/4 + (3 * C1 * CD[-c][CD[-b][MetricPerturbation[-a, -d]]] * CD[d][CD[c][MetricPerturbation[a, b]]])/2 - (3 * C1 * CD[-d][CD[-c][MetricPerturbation[-a, -b]]] * CD[d][CD[c][MetricPerturbation[a, b]]])/4, TheoryName -> "ProjectiveTheorySecondOrder", Method -> "Hard", MaxLaurentDepth -> 1];

==> LstListing/Line109.tex <==
In[109]:= ParticleSpectrum[Coupling1 * CD[-a][ScalarField[]] * CD[a][ScalarField[]], TheoryName -> NotStringTheory, Method -> "Easy", MaxLaurentDepth -> 3]; 

==> LstListing/Line110.tex <==
In[110]:= ParticleSpectrum[Coupling1 * CD[-a][ScalarField[]] * CD[a][ScalarField[]], TheoryName -> "MyVeryCoolTheory", Method -> "InfiniteMonkeys", MaxLaurentDepth -> 3]; 

==> LstListing/Line111.tex <==
In[111]:= ParticleSpectrum[Coupling1 * CD[-a][ScalarField[]] * CD[a][ScalarField[]], TheoryName -> "MyVeryCoolTheory", Method -> "Hard", MaxLaurentDepth -> 4]; 

==> LstListing/Line112.tex <==
In[112]:= ParticleSpectrum[Coupling2 * ScalarField[] + Coupling3 * ScalarField[]^3 + Coupling1 * CD[-a][ScalarField[]] * CD[a][ScalarField[]], TheoryName -> "MyVeryCoolTheory", Method -> "Hard", MaxLaurentDepth -> 3]; 

==> LstListing/Line113.tex <==
In[113]:= DefTensor[Psi[], M4, PrintAs -> "\[Psi]"]; 

==> LstListing/Line114.tex <==
In[114]:= ParticleSpectrum[Coupling1 * CD[-a][ScalarField[]] * CD[a][Psi[]], TheoryName -> "MyVeryCoolTheory", Method -> "Hard", MaxLaurentDepth -> 3]; 

==> LstListing/Line115.tex <==
In[115]:= ParticleSpectrum[Coupling2^2 * ScalarField[]^2 + CD[-a][ScalarField[]] * CD[a][ScalarField[]], TheoryName -> "MyVeryCoolTheory", Method -> "Hard", MaxLaurentDepth -> 3]; 

==> LstListing/Line116.tex <==
In[116]:= ParticleSpectrum[Coupling1 * epsilonG[a, b, c, d] * CD[-a][ScalarField[]] * CD[-b][TwoFormField[-c, -d]], TheoryName -> "MyVeryCoolTheory", Method -> "Hard", MaxLaurentDepth -> 3]; 

==> LstListing/Line28.tex <==
In[#]:= ParticleSpectrum[(Coupling1 * CD[-b][MetricPerturbation[c, -c]] * CD[b][MetricPerturbation[a, -a]])/2 + Coupling2 * CD[-a][MetricPerturbation[a, b]] * CD[-c][MetricPerturbation[-b, c]] - Coupling1 * CD[b][MetricPerturbation[a, -a]] * CD[-c][MetricPerturbation[-b, c]] - (Coupling1 * CD[-c][MetricPerturbation[-a, -b]] * CD[c][MetricPerturbation[a, b]])/2, TheoryName -> "FirstSickFierzPauliTheory", Method -> "Easy", MaxLaurentDepth -> 3]; 

==> LstListing/Line29.tex <==
In[#]:= ParticleSpectrum[Coupling1 * CD[-b][MetricPerturbation[c, -c]] * CD[b][MetricPerturbation[a, -a]] - 2 * Coupling1 * CD[-b][MetricPerturbation[-a, -c]] * CD[c][MetricPerturbation[a, b]] + Coupling1 * CD[-c][MetricPerturbation[-a, -b]] * CD[c][MetricPerturbation[a, b]], TheoryName -> "MarzoTheory", Method -> "Easy", MaxLaurentDepth -> 3]; 

==> LstListing/Line3.tex <==
In[#]:= Print[Names["xAct`PSALTer` * "]]; 

==> LstListing/Line31.tex <==
In[#]:= ParticleSpectrum[-(Coupling1 * CD[-b][CD[-a][MetricPerturbation[a, b]]] * CD[-d][CD[-c][MetricPerturbation[c, d]]]) + 2 * Coupling1 * CD[-b][CD[b][MetricPerturbation[a, -a]]] * CD[-d][CD[-c][MetricPerturbation[c, d]]] - Coupling1 * CD[-b][CD[b][MetricPerturbation[a, -a]]] * CD[-d][CD[d][MetricPerturbation[c, -c]]], TheoryName -> "SquareRicciTheory", Method -> "Easy", MaxLaurentDepth -> 3]; 

==> LstListing/Line32.tex <==
In[#]:= ParticleSpectrum[Coupling2 * CD[-a][ScalarField[]] * CD[a][ScalarField[]] + (Coupling1 * CD[-b][MetricPerturbation[c, -c]] * CD[b][MetricPerturbation[a, -a]])/2 + Coupling1 * CD[-a][MetricPerturbation[a, b]] * CD[-c][MetricPerturbation[-b, c]] - Coupling1 * CD[b][MetricPerturbation[a, -a]] * CD[-c][MetricPerturbation[-b, c]] - (Coupling1 * CD[-c][MetricPerturbation[-a, -b]] * CD[c][MetricPerturbation[a, b]])/2, TheoryName -> "ScalarFierzPauliTheory", Method -> "Easy", MaxLaurentDepth -> 3]; 

==> LstListing/Line36.tex <==
In[#]:= DefConstantSymbol[kLambda, PrintAs -> "\[Lambda]"]; DefConstantSymbol[kR1, PrintAs -> "\!\(\ * SubscriptBox[\(\[ScriptR]\), \(1\)]\)"]; DefConstantSymbol[kR2, PrintAs -> "\!\(\ * SubscriptBox[\(\[ScriptR]\), \(2\)]\)"]; DefConstantSymbol[kR3, PrintAs -> "\!\(\ * SubscriptBox[\(\[ScriptR]\), \(3\)]\)"]; DefConstantSymbol[kR4, PrintAs -> "\!\(\ * SubscriptBox[\(\[ScriptR]\), \(4\)]\)"]; DefConstantSymbol[kR5, PrintAs -> "\!\(\ * SubscriptBox[\(\[ScriptR]\), \(5\)]\)"]; DefConstantSymbol[kR6, PrintAs -> "\!\(\ * SubscriptBox[\(\[ScriptR]\), \(6\)]\)"]; DefConstantSymbol[kT1, PrintAs -> "\!\(\ * SubscriptBox[\(\[ScriptT]\), \(1\)]\)"]; DefConstantSymbol[kT2, PrintAs -> "\!\(\ * SubscriptBox[\(\[ScriptT]\), \(2\)]\)"]; DefConstantSymbol[kT3, PrintAs -> "\!\(\ * SubscriptBox[\(\[ScriptT]\), \(3\)]\)"]; 

==> LstListing/Line38.tex <==
In[#]:= ParticleSpectrum[-(kLambda * SpinConnection[-i, -k, -j] * SpinConnection[i, j, k]) - kLambda * SpinConnection[i, j, -i] * SpinConnection[-j, k, -k] - kLambda * SpinConnection[-i, a, i] * SpinConnection[-k, -a, k] - kLambda * SpinConnection[-i, k, z] * SpinConnection[-k, -z, i] - 2 * kLambda * (*omitted 1161 characters for brevity*) z]] * CD[k][TetradPerturbation[-z, j]])/2 + (kLambda * CD[-k][TetradPerturbation[z, -j]] * CD[k][TetradPerturbation[-z, j]])/2 - kLambda * CD[a][TetradPerturbation[z, -a]] * CD[k][TetradPerturbation[-z, -k]], TheoryName -> "GeneralRelativity", Method -> "Easy", MaxLaurentDepth -> 3];

==> LstListing/Line39.tex <==
In[#]:= ParticleSpectrum[-1/2 * (Alp0 * SpinConnection[-a, -c, -b] * SpinConnection[a, b, c]) - (Alp0 * SpinConnection[a, b, -a] * SpinConnection[-b, c, -c])/2 + 2 * Bet1 * SpinConnection[a, b, -a] * SpinConnection[-b, c, -c] - 2 * Bet1 * SpinConnection[-a, c, d] * SpinConnection[-c, -d, a] - Alp0 * (*omitted 1182 characters for brevity*) b]] * CD[z][TetradPerturbation[-c, -b]] + Bet1 * CD[c][TetradPerturbation[-d, -z]] * CD[z][TetradPerturbation[d, -c]] - Bet1 * CD[c][TetradPerturbation[-z, -d]] * CD[z][TetradPerturbation[d, -c]], TheoryName -> "MinimalEvenScalar", Method -> "Hard", MaxLaurentDepth -> 3];

==> LstListing/Line4.tex <==
In[#]:= Print /@ {Information["M4", LongForm -> False], G[-m, -n], Information["G", LongForm -> False], CD[-a][G[-m, -n]]], Information["CD", LongForm -> False]}; 

==> LstListing/Line40.tex <==
In[#]:= ParticleSpectrum[-1/2 * (Alp0 * SpinConnection[-a, -c, -b] * SpinConnection[a, b, c]) - (Alp0 * SpinConnection[a, b, -a] * SpinConnection[-b, c, -c])/2 + 2 * Bet1 * SpinConnection[a, b, -a] * SpinConnection[-b, c, -c] - 2 * Bet1 * SpinConnection[-a, c, d] * SpinConnection[-c, -d, a] - Alp0 * (*omitted 1690 characters for brevity*) b]] * CD[z][TetradPerturbation[-c, -b]] + Bet1 * CD[c][TetradPerturbation[-d, -z]] * CD[z][TetradPerturbation[d, -c]] - Bet1 * CD[c][TetradPerturbation[-z, -d]] * CD[z][TetradPerturbation[d, -c]], TheoryName -> "MinimalMassiveOddScalar", Method -> "Hard", MaxLaurentDepth -> 3];

==> LstListing/Line41.tex <==
In[#]:= ParticleSpectrum[-2 * Bet1 * SpinConnection[-a, -c, -b] * SpinConnection[a, b, c] - 2 * Bet1 * SpinConnection[-a, c, d] * SpinConnection[-c, -d, a] - 4 * Bet1 * TetradPerturbation[a, b] * CD[-b][SpinConnection[-a, c, -c]] + 4 * Bet1 * CD[-b][SpinConnection[a, b, -a]] + (2 * Alp3 * (*omitted 1571 characters for brevity*) b]] * CD[z][TetradPerturbation[-c, -b]] + Bet1 * CD[c][TetradPerturbation[-d, -z]] * CD[z][TetradPerturbation[d, -c]] - Bet1 * CD[c][TetradPerturbation[-z, -d]] * CD[z][TetradPerturbation[d, -c]], TheoryName -> "MinimalMasslessOddScalar", Method -> "Hard", MaxLaurentDepth -> 3];

==> LstListing/Line43.tex <==
In[#]:= ParticleSpectrum[(2 * kT2 * SpinConnection[-i, k, l] * SpinConnection[-k, -l, i])/3 + (kT2 * SpinConnection[-k, -l, i] * SpinConnection[k, l, -i])/3 - (kR3 * CD[-i][SpinConnection[k, l, -k]] * CD[i][SpinConnection[-l, a, -a]])/2 - kR5 * CD[-i][SpinConnection[k, l, -k]] * CD[i][SpinConnection[-l, (*omitted 2176 characters for brevity*) a, -j]] * CD[l][SpinConnection[j, k, -k]] + (kR3 * CD[-j][SpinConnection[-l, a, -a]] * CD[l][SpinConnection[j, k, -k]])/2 - kR5 * CD[-j][SpinConnection[-l, a, -a]] * CD[l][SpinConnection[j, k, -k]], TheoryName -> StringJoin["Case", ToString[1]], Method -> "Easy", MaxLaurentDepth -> 3];

==> LstListing/Line44.tex <==
In[#]:= ParticleSpectrum[(2 * kT3 * SpinConnection[-i, a, i] * SpinConnection[-k, -a, k])/3 + (2 * kT2 * SpinConnection[-i, k, l] * SpinConnection[-k, -l, i])/3 + (kT2 * SpinConnection[-k, -l, i] * SpinConnection[k, l, -i])/3 - (kR3 * CD[-i][SpinConnection[k, l, -k]] * CD[i][SpinConnection[-l, a, -a]])/2 (*omitted 2808 characters for brevity*) a, -j]] * CD[l][SpinConnection[j, k, -k]] + (kR3 * CD[-j][SpinConnection[-l, a, -a]] * CD[l][SpinConnection[j, k, -k]])/2 - kR5 * CD[-j][SpinConnection[-l, a, -a]] * CD[l][SpinConnection[j, k, -k]], TheoryName -> StringJoin["Case", ToString[2]], Method -> "Easy", MaxLaurentDepth -> 3];

==> LstListing/Line45.tex <==
In[#]:= ParticleSpectrum[-1/3 * (kT1 * SpinConnection[-i, a, i] * SpinConnection[-k, -a, k]) - kT1 * SpinConnection[-i, k, l] * SpinConnection[-k, -l, i] - kR5 * CD[-i][SpinConnection[k, l, -k]] * CD[i][SpinConnection[-l, a, -a]] + (2 * kR2 * CD[b][SpinConnection[j, a, -k]] * CD[-j][SpinConnection[-a, -b, (*omitted 1849 characters for brevity*) l, a]] * CD[-l][SpinConnection[-a, -b, i]])/3 + kR5 * CD[-a][SpinConnection[-l, a, -j]] * CD[l][SpinConnection[j, k, -k]] - kR5 * CD[-j][SpinConnection[-l, a, -a]] * CD[l][SpinConnection[j, k, -k]], TheoryName -> StringJoin["Case", ToString[3]], Method -> "Easy", MaxLaurentDepth -> 3];

==> LstListing/Line46.tex <==
In[#]:= ParticleSpectrum[-1/3 * (kT1 * SpinConnection[-i, a, i] * SpinConnection[-k, -a, k]) - kT1 * SpinConnection[-i, k, l] * SpinConnection[-k, -l, i] - kR5 * CD[-i][SpinConnection[k, l, -k]] * CD[i][SpinConnection[-l, a, -a]] - (2 * kR1 * CD[b][SpinConnection[j, a, -k]] * CD[-j][SpinConnection[-a, -b, (*omitted 1857 characters for brevity*) l, a]] * CD[-l][SpinConnection[-a, -b, i]])/3 + kR5 * CD[-a][SpinConnection[-l, a, -j]] * CD[l][SpinConnection[j, k, -k]] - kR5 * CD[-j][SpinConnection[-l, a, -a]] * CD[l][SpinConnection[j, k, -k]], TheoryName -> StringJoin["Case", ToString[4]], Method -> "Easy", MaxLaurentDepth -> 3];

==> LstListing/Line47.tex <==
In[#]:= ParticleSpectrum[-(kT1 * SpinConnection[-i, a, i] * SpinConnection[-k, -a, k]) - (kT1 * SpinConnection[-i, k, l] * SpinConnection[-k, -l, i])/3 + (kT1 * SpinConnection[-k, -l, i] * SpinConnection[k, l, -i])/3 - kR5 * CD[-i][SpinConnection[k, l, -k]] * CD[i][SpinConnection[-l, a, -a]] - (2 * kR1 * (*omitted 2127 characters for brevity*) l, a]] * CD[-l][SpinConnection[-a, -b, i]])/3 + kR5 * CD[-a][SpinConnection[-l, a, -j]] * CD[l][SpinConnection[j, k, -k]] - kR5 * CD[-j][SpinConnection[-l, a, -a]] * CD[l][SpinConnection[j, k, -k]], TheoryName -> StringJoin["Case", ToString[5]], Method -> "Easy", MaxLaurentDepth -> 3];

==> LstListing/Line48.tex <==
In[#]:= ParticleSpectrum[-1/3 * (kT1 * SpinConnection[-i, a, i] * SpinConnection[-k, -a, k]) - kT1 * SpinConnection[-i, k, l] * SpinConnection[-k, -l, i] - 2 * kR3 * CD[-i][SpinConnection[k, l, -k]] * CD[i][SpinConnection[-l, a, -a]] - kR5 * CD[-i][SpinConnection[k, l, -k]] * CD[i][SpinConnection[-l, a, (*omitted 2489 characters for brevity*) a, -j]] * CD[l][SpinConnection[j, k, -k]] + 2 * kR3 * CD[-j][SpinConnection[-l, a, -a]] * CD[l][SpinConnection[j, k, -k]] - kR5 * CD[-j][SpinConnection[-l, a, -a]] * CD[l][SpinConnection[j, k, -k]], TheoryName -> StringJoin["Case", ToString[6]], Method -> "Easy", MaxLaurentDepth -> 3];

==> LstListing/Line49.tex <==
In[#]:= ParticleSpectrum[-1/3 * (kT1 * SpinConnection[-i, a, i] * SpinConnection[-k, -a, k]) - kT1 * SpinConnection[-i, k, l] * SpinConnection[-k, -l, i] + 2 * kR1 * CD[-i][SpinConnection[k, l, -k]] * CD[i][SpinConnection[-l, a, -a]] - 2 * kR3 * CD[-i][SpinConnection[k, l, -k]] * CD[i][SpinConnection[-l, (*omitted 3057 characters for brevity*) a, -a]] * CD[l][SpinConnection[j, k, -k]] + 2 * kR3 * CD[-j][SpinConnection[-l, a, -a]] * CD[l][SpinConnection[j, k, -k]] - kR5 * CD[-j][SpinConnection[-l, a, -a]] * CD[l][SpinConnection[j, k, -k]], TheoryName -> StringJoin["Case", ToString[7]], Method -> "Easy", MaxLaurentDepth -> 3];

==> LstListing/Line5.tex <==
In[#]:= Print[IndicesOfVBundle[TangentM4]]; 

==> LstListing/Line50.tex <==
In[#]:= ParticleSpectrum[(2 * kT3 * SpinConnection[-i, a, i] * SpinConnection[-k, -a, k])/3 - kR5 * CD[-i][SpinConnection[k, l, -k]] * CD[i][SpinConnection[-l, a, -a]] - (2 * kR1 * CD[b][SpinConnection[j, a, -k]] * CD[-j][SpinConnection[-a, -b, k]])/3 - (2 * kR1 * CD[-j][SpinConnection[-a, -b, k]] * (*omitted 1260 characters for brevity*) l, a]] * CD[-l][SpinConnection[-a, -b, i]])/3 + kR5 * CD[-a][SpinConnection[-l, a, -j]] * CD[l][SpinConnection[j, k, -k]] - kR5 * CD[-j][SpinConnection[-l, a, -a]] * CD[l][SpinConnection[j, k, -k]], TheoryName -> StringJoin["Case", ToString[8]], Method -> "Easy", MaxLaurentDepth -> 3];

==> LstListing/Line51.tex <==
In[#]:= ParticleSpectrum[-(kR5 * CD[-i][SpinConnection[k, l, -k]] * CD[i][SpinConnection[-l, a, -a]]) - (2 * kR1 * CD[b][SpinConnection[j, a, -k]] * CD[-j][SpinConnection[-a, -b, k]])/3 - (2 * kR1 * CD[-j][SpinConnection[-a, -b, k]] * CD[-k][SpinConnection[a, b, j]])/3 + (2 * kR1 * CD[-j][SpinConnection[-a, -b, k]] * CD[-k][SpinConnection[j, a, b]])/3 - kR5 * CD[-a][SpinConnection[-l, a, -j]] * CD[-k][SpinConnection[j, k, l]] + kR5 * CD[-j][SpinConnection[-l, a, -a]] * CD[-k][SpinConnection[j, k, l]] - kR5 * CD[-a][SpinConnection[-l, a, -j]] * CD[-k][SpinConnection[k, l, j]] + 2 * kR5 * CD[-j][SpinConnection[-l, a, -a]] * CD[-k][SpinConnection[k, l, j]] + (2 * kR1 * CD[-k][SpinConnection[a, b, j]] * CD[k][SpinConnection[-a, -b, -j]])/3 - (2 * kR1 * CD[-k][SpinConnection[j, a, b]] * CD[k][SpinConnection[-a, -b, -j]])/3 + (2 * kR1 * CD[b][SpinConnection[-i, a, l]] * CD[-l][SpinConnection[-a, -b, i]])/3 - (8 * kR1 * CD[b][SpinConnection[-i, l, a]] * CD[-l][SpinConnection[-a, -b, i]])/3 + kR5 * CD[-a][SpinConnection[-l, a, -j]] * CD[l][SpinConnection[j, k, -k]] - kR5 * CD[-j][SpinConnection[-l, a, -a]] * CD[l][SpinConnection[j, k, -k]], TheoryName -> StringJoin["Case", ToString[9]], Method -> "Easy", MaxLaurentDepth -> 3]; 

==> LstListing/Line52.tex <==
In[#]:= ParticleSpectrum[-1/2 * (kR3 * CD[-i][SpinConnection[k, l, -k]] * CD[i][SpinConnection[-l, a, -a]]) - kR5 * CD[-i][SpinConnection[k, l, -k]] * CD[i][SpinConnection[-l, a, -a]] + (kR3 * CD[-a][SpinConnection[-l, a, -j]] * CD[-k][SpinConnection[j, k, l]])/2 - kR5 * CD[-a][SpinConnection[-l, a, -j]] * CD[-k][SpinConnection[j, k, l]] - (kR3 * CD[-j][SpinConnection[-l, a, -a]] * CD[-k][SpinConnection[j, k, l]])/2 + kR5 * CD[-j][SpinConnection[-l, a, -a]] * CD[-k][SpinConnection[j, k, l]] - (kR3 * CD[-a][SpinConnection[-l, a, -j]] * CD[-k][SpinConnection[k, l, j]])/2 - kR5 * CD[-a][SpinConnection[-l, a, -j]] * CD[-k][SpinConnection[k, l, j]] + kR3 * CD[-j][SpinConnection[-l, a, -a]] * CD[-k][SpinConnection[k, l, j]] + 2 * kR5 * CD[-j][SpinConnection[-l, a, -a]] * CD[-k][SpinConnection[k, l, j]] - 4 * kR3 * CD[b][SpinConnection[-i, l, a]] * CD[-l][SpinConnection[-a, -b, i]] - (kR3 * CD[-a][SpinConnection[-l, a, -j]] * CD[l][SpinConnection[j, k, -k]])/2 + kR5 * CD[-a][SpinConnection[-l, a, -j]] * CD[l][SpinConnection[j, k, -k]] + (kR3 * CD[-j][SpinConnection[-l, a, -a]] * CD[l][SpinConnection[j, k, -k]])/2 - kR5 * CD[-j][SpinConnection[-l, a, -a]] * CD[l][SpinConnection[j, k, -k]], TheoryName -> StringJoin["Case", ToString[10]], Method -> "Easy", MaxLaurentDepth -> 3]; 

==> LstListing/Line53.tex <==
In[#]:= ParticleSpectrum[-1/2 * (kR3 * CD[-i][SpinConnection[k, l, -k]] * CD[i][SpinConnection[-l, a, -a]]) - kR5 * CD[-i][SpinConnection[k, l, -k]] * CD[i][SpinConnection[-l, a, -a]] + (2 * kR2 * CD[b][SpinConnection[j, a, -k]] * CD[-j][SpinConnection[-a, -b, k]])/3 - (kR2 * CD[-j][SpinConnection[-a, -b, (*omitted 1262 characters for brevity*) a, -j]] * CD[l][SpinConnection[j, k, -k]] + (kR3 * CD[-j][SpinConnection[-l, a, -a]] * CD[l][SpinConnection[j, k, -k]])/2 - kR5 * CD[-j][SpinConnection[-l, a, -a]] * CD[l][SpinConnection[j, k, -k]], TheoryName -> StringJoin["Case", ToString[11]], Method -> "Easy", MaxLaurentDepth -> 3];

==> LstListing/Line54.tex <==
In[#]:= ParticleSpectrum[(2 * kT2 * SpinConnection[-i, k, l] * SpinConnection[-k, -l, i])/3 + (kT2 * SpinConnection[-k, -l, i] * SpinConnection[k, l, -i])/3 - (kR3 * CD[-i][SpinConnection[k, l, -k]] * CD[i][SpinConnection[-l, a, -a]])/2 - kR5 * CD[-i][SpinConnection[k, l, -k]] * CD[i][SpinConnection[-l, (*omitted 1597 characters for brevity*) a, -j]] * CD[l][SpinConnection[j, k, -k]] + (kR3 * CD[-j][SpinConnection[-l, a, -a]] * CD[l][SpinConnection[j, k, -k]])/2 - kR5 * CD[-j][SpinConnection[-l, a, -a]] * CD[l][SpinConnection[j, k, -k]], TheoryName -> StringJoin["Case", ToString[12]], Method -> "Easy", MaxLaurentDepth -> 3];

==> LstListing/Line55.tex <==
In[#]:= ParticleSpectrum[2 * kR1 * CD[-i][SpinConnection[k, l, -k]] * CD[i][SpinConnection[-l, a, -a]] - 2 * kR3 * CD[-i][SpinConnection[k, l, -k]] * CD[i][SpinConnection[-l, a, -a]] - kR5 * CD[-i][SpinConnection[k, l, -k]] * CD[i][SpinConnection[-l, a, -a]] - (2 * kR1 * CD[b][SpinConnection[j, a, -k]] * (*omitted 1829 characters for brevity*) a, -a]] * CD[l][SpinConnection[j, k, -k]] + 2 * kR3 * CD[-j][SpinConnection[-l, a, -a]] * CD[l][SpinConnection[j, k, -k]] - kR5 * CD[-j][SpinConnection[-l, a, -a]] * CD[l][SpinConnection[j, k, -k]], TheoryName -> StringJoin["Case", ToString[13]], Method -> "Easy", MaxLaurentDepth -> 3];

==> LstListing/Line56.tex <==
In[#]:= ParticleSpectrum[(2 * kT3 * SpinConnection[-i, a, i] * SpinConnection[-k, -a, k])/3 - (kR3 * CD[-i][SpinConnection[k, l, -k]] * CD[i][SpinConnection[-l, a, -a]])/2 - kR5 * CD[-i][SpinConnection[k, l, -k]] * CD[i][SpinConnection[-l, a, -a]] + (kR3 * CD[-a][SpinConnection[-l, a, -j]] * (*omitted 1309 characters for brevity*) a, -j]] * CD[l][SpinConnection[j, k, -k]] + (kR3 * CD[-j][SpinConnection[-l, a, -a]] * CD[l][SpinConnection[j, k, -k]])/2 - kR5 * CD[-j][SpinConnection[-l, a, -a]] * CD[l][SpinConnection[j, k, -k]], TheoryName -> StringJoin["Case", ToString[14]], Method -> "Easy", MaxLaurentDepth -> 3];

==> LstListing/Line57.tex <==
In[#]:= ParticleSpectrum[(2 * kT3 * SpinConnection[-i, a, i] * SpinConnection[-k, -a, k])/3 + (2 * kT2 * SpinConnection[-i, k, l] * SpinConnection[-k, -l, i])/3 + (kT2 * SpinConnection[-k, -l, i] * SpinConnection[k, l, -i])/3 - (kR3 * CD[-i][SpinConnection[k, l, -k]] * CD[i][SpinConnection[-l, a, -a]])/2 (*omitted 2229 characters for brevity*) a, -j]] * CD[l][SpinConnection[j, k, -k]] + (kR3 * CD[-j][SpinConnection[-l, a, -a]] * CD[l][SpinConnection[j, k, -k]])/2 - kR5 * CD[-j][SpinConnection[-l, a, -a]] * CD[l][SpinConnection[j, k, -k]], TheoryName -> StringJoin["Case", ToString[15]], Method -> "Easy", MaxLaurentDepth -> 3];

==> LstListing/Line58.tex <==
In[#]:= ParticleSpectrum[(2 * kT3 * SpinConnection[-i, a, i] * SpinConnection[-k, -a, k])/3 - (kR3 * CD[-i][SpinConnection[k, l, -k]] * CD[i][SpinConnection[-l, a, -a]])/2 - kR5 * CD[-i][SpinConnection[k, l, -k]] * CD[i][SpinConnection[-l, a, -a]] + (2 * kR2 * CD[b][SpinConnection[j, a, -k]] * (*omitted 1889 characters for brevity*) a, -j]] * CD[l][SpinConnection[j, k, -k]] + (kR3 * CD[-j][SpinConnection[-l, a, -a]] * CD[l][SpinConnection[j, k, -k]])/2 - kR5 * CD[-j][SpinConnection[-l, a, -a]] * CD[l][SpinConnection[j, k, -k]], TheoryName -> StringJoin["Case", ToString[16]], Method -> "Easy", MaxLaurentDepth -> 3];

==> LstListing/Line59.tex <==
In[#]:= ParticleSpectrum[-1/3 * (kT1 * SpinConnection[-i, a, i] * SpinConnection[-k, -a, k]) - kT1 * SpinConnection[-i, k, l] * SpinConnection[-k, -l, i] - kR5 * CD[-i][SpinConnection[k, l, -k]] * CD[i][SpinConnection[-l, a, -a]] - kR5 * CD[-a][SpinConnection[-l, a, -j]] * CD[-k][SpinConnection[j, k, l]] (*omitted 1270 characters for brevity*) -a]] * CD[k][TetradPerturbation[-l, -k]])/3 + kR5 * CD[-a][SpinConnection[-l, a, -j]] * CD[l][SpinConnection[j, k, -k]] - kR5 * CD[-j][SpinConnection[-l, a, -a]] * CD[l][SpinConnection[j, k, -k]], TheoryName -> StringJoin["Case", ToString[17]], Method -> "Easy", MaxLaurentDepth -> 3];

==> LstListing/Line6.tex <==
In[#]:= Print /@ {V[-m], Information["V", LongForm -> False], P[-m], Information["P", LongForm -> False], Def, Information["Def", LongForm -> False], En, Information["En", LongForm -> False], Mo, Information["Mo", LongForm -> False]}; 

==> LstListing/Line60.tex <==
In[#]:= ParticleSpectrum[-(kT1 * SpinConnection[-i, a, i] * SpinConnection[-k, -a, k]) - (kT1 * SpinConnection[-i, k, l] * SpinConnection[-k, -l, i])/3 + (kT1 * SpinConnection[-k, -l, i] * SpinConnection[k, l, -i])/3 - kR5 * CD[-i][SpinConnection[k, l, -k]] * CD[i][SpinConnection[-l, a, -a]] - kR5 * (*omitted 1540 characters for brevity*) -a]] * CD[k][TetradPerturbation[-l, -k]] + kR5 * CD[-a][SpinConnection[-l, a, -j]] * CD[l][SpinConnection[j, k, -k]] - kR5 * CD[-j][SpinConnection[-l, a, -a]] * CD[l][SpinConnection[j, k, -k]], TheoryName -> StringJoin["Case", ToString[18]], Method -> "Easy", MaxLaurentDepth -> 3];

==> LstListing/Line61.tex <==
In[#]:= ParticleSpectrum[-1/3 * (kT1 * SpinConnection[-i, a, i] * SpinConnection[-k, -a, k]) - kT1 * SpinConnection[-i, k, l] * SpinConnection[-k, -l, i] - 2 * kR3 * CD[-i][SpinConnection[k, l, -k]] * CD[i][SpinConnection[-l, a, -a]] - kR5 * CD[-i][SpinConnection[k, l, -k]] * CD[i][SpinConnection[-l, a, (*omitted 1910 characters for brevity*) a, -j]] * CD[l][SpinConnection[j, k, -k]] + 2 * kR3 * CD[-j][SpinConnection[-l, a, -a]] * CD[l][SpinConnection[j, k, -k]] - kR5 * CD[-j][SpinConnection[-l, a, -a]] * CD[l][SpinConnection[j, k, -k]], TheoryName -> StringJoin["Case", ToString[19]], Method -> "Easy", MaxLaurentDepth -> 3];

==> LstListing/Line67.tex <==
In[#]:= ParticleSpectrum[-1/2 * (A0 * Connection[a, b, c] * Connection[-b, -c, -a]) + (A0 * Connection[a, -a, b] * Connection[c, -b, -c])/2 - (A0 * MetricPerturbation[c, -c] * CD[-b][Connection[a, -a, b]])/4 + (A0 * MetricPerturbation[c, -c] * CD[-b][Connection[a, b, -a]])/4 - (A0 * MetricPerturbation[-a, -c] * CD[-b][Connection[a, b, c]])/2 - (A0 * Connection[a, b, c] * CD[-b][MetricPerturbation[-a, -c]])/2 - (A0 * Connection[a, -a, b] * CD[-b][MetricPerturbation[c, -c]])/4 + (A0 * Connection[a, b, -a] * CD[-b][MetricPerturbation[c, -c]])/4 + (A0 * MetricPerturbation[a, b] * CD[-b][CD[-a][MetricPerturbation[c, -c]]])/2 - (A0 * CD[-b][MetricPerturbation[c, -c]] * CD[b][MetricPerturbation[a, -a]])/8 + (A0 * Connection[a, -a, b] * CD[-c][MetricPerturbation[-b, c]])/2 - (A0 * CD[-a][MetricPerturbation[a, b]] * CD[-c][MetricPerturbation[-b, c]])/2 + (A0 * CD[b][MetricPerturbation[a, -a]] * CD[-c][MetricPerturbation[-b, c]])/2 - A0 * MetricPerturbation[a, b] * CD[-c][CD[-b][MetricPerturbation[-a, c]]] + (A0 * MetricPerturbation[a, -a] * CD[-c][CD[-b][MetricPerturbation[b, c]]])/4 + (A0 * MetricPerturbation[a, b] * CD[-c][CD[c][MetricPerturbation[-a, -b]]])/2 - (A0 * MetricPerturbation[a, -a] * CD[-c][CD[c][MetricPerturbation[b, -b]]])/4 + (A0 * MetricPerturbation[-b, -c] * CD[c][Connection[a, -a, b]])/2 - (A0 * CD[-b][MetricPerturbation[-a, -c]] * CD[c][MetricPerturbation[a, b]])/4 + (3 * A0 * CD[-c][MetricPerturbation[-a, -b]] * CD[c][MetricPerturbation[a, b]])/8, TheoryName -> "MetricAffineEinsteinHilbertTheorySecondOrder", Method -> "Hard", MaxLaurentDepth -> 3]; 

==> LstListing/Line68.tex <==
In[#]:= ParticleSpectrum[((-2 * A0 + 2 * A1 + A2 - 12 * A6 + 2 * A9) * Connection[-a, m, -m] * Connection[a, b, -b])/6 + ((-A0 + 2 * (-4 * A1 + A5 + 9 * A7 - 2 * A9)) * Connection[-a, -b, -m] * Connection[a, b, m])/8 + ((-A0 + 2 * (-2 * A2 + A5 + 9 * A7 - 2 * A9)) * Connection[-a, -m, -b] * Connection[a, (*omitted 1808 characters for brevity*) n, -n]] * CD[m][Connection[a, b, -b]] - (A0 * CD[-b][MetricPerturbation[-a, -m]] * CD[m][MetricPerturbation[a, b]])/4 + (A0 * CD[-m][MetricPerturbation[-a, -b]] * CD[m][MetricPerturbation[a, b]])/8, TheoryName -> "IsoWeylTheorySecondOrder", Method -> "Hard", MaxLaurentDepth -> 1];

==> LstListing/Line69.tex <==
In[#]:= ParticleSpectrum[((4 * A1 + 2 * A2 + 3 * A3 - 12 * A6 + 2 * A9) * Connection[-a, c, -c] * Connection[a, b, -b])/6 + ((-A0 - 6 * A1 - A2 - 3 * A3 + 8 * A6 + 4 * A7 - 2 * A9) * Connection[-a, -b, -c] * Connection[a, b, c])/4 + ((-A0 - 2 * A1 - 3 * A2 - 3 * A3 + 8 * A6 + 4 * A7 - 2 * A9) * (*omitted 3235 characters for brevity*) b, c]] + C1 * CD[-c][CD[-b][MetricPerturbation[-a, -m]]] * CD[m][CD[c][MetricPerturbation[a, b]]] - C1 * CD[-m][CD[-b][MetricPerturbation[-a, -c]]] * CD[m][CD[c][MetricPerturbation[a, b]]], TheoryName -> "ExtendedProjectiveTheorySecondOrder", Method -> "Hard", MaxLaurentDepth -> 1];

==> LstListing/Line7.tex <==
In[#]:= Print /@ {Information["DefField", LongForm -> False], Information["ParticleSpectrum", LongForm -> False]}; 

==> LstListing/Line71.tex <==
In[#]:= ParticleSpectrum[-1/2 * (A0 * Connection[a, b, c] * Connection[-b, -c, -a]) + (A0 * Connection[a, -a, b] * Connection[c, -b, -c])/2 - (A0 * MetricPerturbation[c, -c] * CD[-b][Connection[a, -a, b]])/4 + (A0 * MetricPerturbation[c, -c] * CD[-b][Connection[a, b, -a]])/4 - (A0 * MetricPerturbation[-a, (*omitted 8137 characters for brevity*) b]]])/4 + (3 * C1 * CD[-c][CD[-b][MetricPerturbation[-a, -d]]] * CD[d][CD[c][MetricPerturbation[a, b]]])/2 - (3 * C1 * CD[-d][CD[-c][MetricPerturbation[-a, -b]]] * CD[d][CD[c][MetricPerturbation[a, b]]])/4, TheoryName -> "ProjectiveTheorySecondOrder", Method -> "Hard", MaxLaurentDepth -> 1];

==> LstListing/Line72.tex <==
In[#]:= ParticleSpectrum[Coupling1 * CD[-a][ScalarField[]] * CD[a][ScalarField[]], TheoryName -> NotStringTheory, Method -> "Easy", MaxLaurentDepth -> 3]; 

==> LstListing/Line73.tex <==
In[#]:= ParticleSpectrum[Coupling1 * CD[-a][ScalarField[]] * CD[a][ScalarField[]], TheoryName -> "MyVeryCoolTheory", Method -> "InfiniteMonkeys", MaxLaurentDepth -> 3]; 

==> LstListing/Line74.tex <==
In[#]:= ParticleSpectrum[Coupling1 * CD[-a][ScalarField[]] * CD[a][ScalarField[]], TheoryName -> "MyVeryCoolTheory", Method -> "Hard", MaxLaurentDepth -> 4]; 

==> LstListing/Line75.tex <==
In[#]:= ParticleSpectrum[Coupling2 * ScalarField[] + Coupling3 * ScalarField[]^3 + Coupling1 * CD[-a][ScalarField[]] * CD[a][ScalarField[]], TheoryName -> "MyVeryCoolTheory", Method -> "Hard", MaxLaurentDepth -> 3]; 

==> LstListing/Line76.tex <==
In[#]:= DefTensor[Psi[], M4, PrintAs -> "\[Psi]"]; 

==> LstListing/Line77.tex <==
In[#]:= ParticleSpectrum[Coupling1 * CD[-a][ScalarField[]] * CD[a][Psi[]], TheoryName -> "MyVeryCoolTheory", Method -> "Hard", MaxLaurentDepth -> 3]; 

==> LstListing/Line78.tex <==
In[#]:= ParticleSpectrum[Coupling2^2 * ScalarField[]^2 + CD[-a][ScalarField[]] * CD[a][ScalarField[]], TheoryName -> "MyVeryCoolTheory", Method -> "Hard", MaxLaurentDepth -> 3]; 

==> LstListing/Line79.tex <==
In[#]:= ParticleSpectrum[Coupling1 * epsilonG[a, b, c, d] * CD[-a][ScalarField[]] * CD[-b][TwoFormField[-c, -d]], TheoryName -> "MyVeryCoolTheory", Method -> "Hard", MaxLaurentDepth -> 3]; 

==> LstListing/Line8.tex <==
In[#]:= Print /@ {Information["PrintSourceAs", LongForm -> False], Information["TheoryName", LongForm -> False], Information["MaxLaurentDepth", LongForm -> False]}; 

==> LstListing/Line80.tex <==
In[80]:= ParticleSpectrum[-1/3 * (kT1 * SpinConnection[-i, a, i] * SpinConnection[-k, -a, k]) - (kT1 * SpinConnection[-i, k, l] * SpinConnection[-k, -l, i])/3 + (2 * kT2 * SpinConnection[-i, k, l] * SpinConnection[-k, -l, i])/3 + (kT1 * SpinConnection[-k, -l, i] * SpinConnection[k, l, -i])/3 + (kT2 * (*omitted 2938 characters for brevity*) l, a]] * CD[-l][SpinConnection[-a, -b, i]] - 4 * kR3 * CD[-a][SpinConnection[-l, a, -j]] * CD[l][SpinConnection[j, k, -k]] + 4 * kR3 * CD[-j][SpinConnection[-l, a, -a]] * CD[l][SpinConnection[j, k, -k]], TheoryName -> StringJoin["Case", ToString[38]], Method -> "Easy", MaxLaurentDepth -> 3];

==> LstListing/Line81.tex <==
In[81]:= ParticleSpectrum[-1/3 * (kT1 * SpinConnection[-i, a, i] * SpinConnection[-k, -a, k]) - kT1 * SpinConnection[-i, k, l] * SpinConnection[-k, -l, i] + (2 * kR2 * CD[b][SpinConnection[j, a, -k]] * CD[-j][SpinConnection[-a, -b, k]])/3 - (kR2 * CD[-j][SpinConnection[-a, -b, k]] * (*omitted 1714 characters for brevity*) l, a]] * CD[-l][SpinConnection[-a, -b, i]] - 4 * kR3 * CD[-a][SpinConnection[-l, a, -j]] * CD[l][SpinConnection[j, k, -k]] + 4 * kR3 * CD[-j][SpinConnection[-l, a, -a]] * CD[l][SpinConnection[j, k, -k]], TheoryName -> StringJoin["Case", ToString[39]], Method -> "Easy", MaxLaurentDepth -> 3];

==> LstListing/Line82.tex <==
In[82]:= ParticleSpectrum[(2 * kT2 * SpinConnection[-i, k, l] * SpinConnection[-k, -l, i])/3 + (kT2 * SpinConnection[-k, -l, i] * SpinConnection[k, l, -i])/3 + (2 * kR2 * CD[b][SpinConnection[j, a, -k]] * CD[-j][SpinConnection[-a, -b, k]])/3 - (kR2 * CD[-j][SpinConnection[-a, -b, k]] * (*omitted 1405 characters for brevity*) l, a]] * CD[-l][SpinConnection[-a, -b, i]] - 2 * kR4 * CD[-a][SpinConnection[-l, a, -j]] * CD[l][SpinConnection[j, k, -k]] + 2 * kR4 * CD[-j][SpinConnection[-l, a, -a]] * CD[l][SpinConnection[j, k, -k]], TheoryName -> StringJoin["Case", ToString[40]], Method -> "Easy", MaxLaurentDepth -> 3];

==> LstListing/Line83.tex <==
In[83]:= ParticleSpectrum[(2 * kT3 * SpinConnection[-i, a, i] * SpinConnection[-k, -a, k])/3 + (2 * kT2 * SpinConnection[-i, k, l] * SpinConnection[-k, -l, i])/3 + (kT2 * SpinConnection[-k, -l, i] * SpinConnection[k, l, -i])/3 + (2 * kR2 * CD[b][SpinConnection[j, a, -k]] * CD[-j][SpinConnection[-a, -b, (*omitted 2021 characters for brevity*) l, a]] * CD[-l][SpinConnection[-a, -b, i]] - kR3 * CD[-a][SpinConnection[-l, a, -j]] * CD[l][SpinConnection[j, k, -k]] + kR3 * CD[-j][SpinConnection[-l, a, -a]] * CD[l][SpinConnection[j, k, -k]], TheoryName -> StringJoin["Case", ToString[41]], Method -> "Easy", MaxLaurentDepth -> 3];

==> LstListing/Line84.tex <==
In[84]:= ParticleSpectrum[-1/3 * (kT1 * SpinConnection[-i, a, i] * SpinConnection[-k, -a, k]) + (2 * kT3 * SpinConnection[-i, a, i] * SpinConnection[-k, -a, k])/3 - kT1 * SpinConnection[-i, k, l] * SpinConnection[-k, -l, i] - kR5 * CD[-i][SpinConnection[k, l, -k]] * CD[i][SpinConnection[-l, a, -a]] + (2 * (*omitted 2482 characters for brevity*) l, a]] * CD[-l][SpinConnection[-a, -b, i]])/3 + kR5 * CD[-a][SpinConnection[-l, a, -j]] * CD[l][SpinConnection[j, k, -k]] - kR5 * CD[-j][SpinConnection[-l, a, -a]] * CD[l][SpinConnection[j, k, -k]], TheoryName -> StringJoin["Case", ToString[42]], Method -> "Easy", MaxLaurentDepth -> 3];

==> LstListing/Line85.tex <==
In[85]:= ParticleSpectrum[-(kT1 * SpinConnection[-i, a, i] * SpinConnection[-k, -a, k]) - (kT1 * SpinConnection[-i, k, l] * SpinConnection[-k, -l, i])/3 + (2 * kT2 * SpinConnection[-i, k, l] * SpinConnection[-k, -l, i])/3 + (kT1 * SpinConnection[-k, -l, i] * SpinConnection[k, l, -i])/3 + (kT2 * (*omitted 3040 characters for brevity*) l, a]] * CD[-l][SpinConnection[-a, -b, i]])/3 + kR5 * CD[-a][SpinConnection[-l, a, -j]] * CD[l][SpinConnection[j, k, -k]] - kR5 * CD[-j][SpinConnection[-l, a, -a]] * CD[l][SpinConnection[j, k, -k]], TheoryName -> StringJoin["Case", ToString[43]], Method -> "Easy", MaxLaurentDepth -> 3];

==> LstListing/Line86.tex <==
In[86]:= ParticleSpectrum[-1/3 * (kT1 * SpinConnection[-i, a, i] * SpinConnection[-k, -a, k]) + (2 * kT3 * SpinConnection[-i, a, i] * SpinConnection[-k, -a, k])/3 - kT1 * SpinConnection[-i, k, l] * SpinConnection[-k, -l, i] - kR5 * CD[-i][SpinConnection[k, l, -k]] * CD[i][SpinConnection[-l, a, -a]] - (2 * (*omitted 2490 characters for brevity*) l, a]] * CD[-l][SpinConnection[-a, -b, i]])/3 + kR5 * CD[-a][SpinConnection[-l, a, -j]] * CD[l][SpinConnection[j, k, -k]] - kR5 * CD[-j][SpinConnection[-l, a, -a]] * CD[l][SpinConnection[j, k, -k]], TheoryName -> StringJoin["Case", ToString[44]], Method -> "Easy", MaxLaurentDepth -> 3];

==> LstListing/Line87.tex <==
In[87]:= ParticleSpectrum[-(kT1 * SpinConnection[-i, a, i] * SpinConnection[-k, -a, k]) - (kT1 * SpinConnection[-i, k, l] * SpinConnection[-k, -l, i])/3 + (2 * kT2 * SpinConnection[-i, k, l] * SpinConnection[-k, -l, i])/3 + (kT1 * SpinConnection[-k, -l, i] * SpinConnection[k, l, -i])/3 + (kT2 * (*omitted 3048 characters for brevity*) l, a]] * CD[-l][SpinConnection[-a, -b, i]])/3 + kR5 * CD[-a][SpinConnection[-l, a, -j]] * CD[l][SpinConnection[j, k, -k]] - kR5 * CD[-j][SpinConnection[-l, a, -a]] * CD[l][SpinConnection[j, k, -k]], TheoryName -> StringJoin["Case", ToString[45]], Method -> "Easy", MaxLaurentDepth -> 3];

==> LstListing/Line88.tex <==
In[88]:= ParticleSpectrum[-(kT1 * SpinConnection[-i, a, i] * SpinConnection[-k, -a, k]) - (kT1 * SpinConnection[-i, k, l] * SpinConnection[-k, -l, i])/3 + (2 * kT2 * SpinConnection[-i, k, l] * SpinConnection[-k, -l, i])/3 + (kT1 * SpinConnection[-k, -l, i] * SpinConnection[k, l, -i])/3 + (kT2 * (*omitted 3652 characters for brevity*) l, a]] * CD[-l][SpinConnection[-a, -b, i]])/3 - 2 * kR1 * CD[-a][SpinConnection[-l, a, -j]] * CD[l][SpinConnection[j, k, -k]] + 2 * kR1 * CD[-j][SpinConnection[-l, a, -a]] * CD[l][SpinConnection[j, k, -k]], TheoryName -> StringJoin["Case", ToString[46]], Method -> "Easy", MaxLaurentDepth -> 3];

==> LstListing/Line89.tex <==
In[89]:= ParticleSpectrum[-1/3 * (kT1 * SpinConnection[-i, a, i] * SpinConnection[-k, -a, k]) + (2 * kT3 * SpinConnection[-i, a, i] * SpinConnection[-k, -a, k])/3 - kT1 * SpinConnection[-i, k, l] * SpinConnection[-k, -l, i] - kR5 * CD[-i][SpinConnection[k, l, -k]] * CD[i][SpinConnection[-l, a, -a]] - kR5 * (*omitted 1902 characters for brevity*) -a]] * CD[k][TetradPerturbation[-l, -k]])/3 + kR5 * CD[-a][SpinConnection[-l, a, -j]] * CD[l][SpinConnection[j, k, -k]] - kR5 * CD[-j][SpinConnection[-l, a, -a]] * CD[l][SpinConnection[j, k, -k]], TheoryName -> StringJoin["Case", ToString[47]], Method -> "Easy", MaxLaurentDepth -> 3];

==> LstListing/Line9.tex <==
In[#]:= SetOptions[$FrontEndSession, EvaluationCompletionAction -> "ScrollToOutput"]; $DefInfoQ = False; Unprotect[AutomaticRules]; Options[AutomaticRules] = {Verbose -> False}; Protect[AutomaticRules]; 

==> LstListing/Line90.tex <==
In[90]:= ParticleSpectrum[-(kT1 * SpinConnection[-i, a, i] * SpinConnection[-k, -a, k]) - (kT1 * SpinConnection[-i, k, l] * SpinConnection[-k, -l, i])/3 + (2 * kT2 * SpinConnection[-i, k, l] * SpinConnection[-k, -l, i])/3 + (kT1 * SpinConnection[-k, -l, i] * SpinConnection[k, l, -i])/3 + (kT2 * (*omitted 2460 characters for brevity*) -a]] * CD[k][TetradPerturbation[-l, -k]] + kR5 * CD[-a][SpinConnection[-l, a, -j]] * CD[l][SpinConnection[j, k, -k]] - kR5 * CD[-j][SpinConnection[-l, a, -a]] * CD[l][SpinConnection[j, k, -k]], TheoryName -> StringJoin["Case", ToString[48]], Method -> "Easy", MaxLaurentDepth -> 3];

==> LstListing/Line91.tex <==
In[91]:= ParticleSpectrum[-(kT1 * SpinConnection[-i, a, i] * SpinConnection[-k, -a, k]) - kT1 * SpinConnection[-i, k, l] * SpinConnection[-k, -l, i] - kR5 * CD[-i][SpinConnection[k, l, -k]] * CD[i][SpinConnection[-l, a, -a]] + (2 * kR2 * CD[b][SpinConnection[j, a, -k]] * CD[-j][SpinConnection[-a, -b, (*omitted 1816 characters for brevity*) l, a]] * CD[-l][SpinConnection[-a, -b, i]])/3 + kR5 * CD[-a][SpinConnection[-l, a, -j]] * CD[l][SpinConnection[j, k, -k]] - kR5 * CD[-j][SpinConnection[-l, a, -a]] * CD[l][SpinConnection[j, k, -k]], TheoryName -> StringJoin["Case", ToString[49]], Method -> "Easy", MaxLaurentDepth -> 3];

==> LstListing/Line92.tex <==
In[92]:= ParticleSpectrum[-1/3 * (kT1 * SpinConnection[-i, a, i] * SpinConnection[-k, -a, k]) + (2 * kT3 * SpinConnection[-i, a, i] * SpinConnection[-k, -a, k])/3 - kT1 * SpinConnection[-i, k, l] * SpinConnection[-k, -l, i] + kR1 * CD[-i][SpinConnection[k, l, -k]] * CD[i][SpinConnection[-l, a, -a]] - (2 * (*omitted 2490 characters for brevity*) l, a]] * CD[-l][SpinConnection[-a, -b, i]])/3 - kR1 * CD[-a][SpinConnection[-l, a, -j]] * CD[l][SpinConnection[j, k, -k]] + kR1 * CD[-j][SpinConnection[-l, a, -a]] * CD[l][SpinConnection[j, k, -k]], TheoryName -> StringJoin["Case", ToString[50]], Method -> "Easy", MaxLaurentDepth -> 3];

==> LstListing/Line93.tex <==
In[93]:= ParticleSpectrum[-(kT1 * SpinConnection[-i, a, i] * SpinConnection[-k, -a, k]) - (kT1 * SpinConnection[-i, k, l] * SpinConnection[-k, -l, i])/3 + (2 * kT2 * SpinConnection[-i, k, l] * SpinConnection[-k, -l, i])/3 + (kT1 * SpinConnection[-k, -l, i] * SpinConnection[k, l, -i])/3 + (kT2 * (*omitted 3072 characters for brevity*) l, a]] * CD[-l][SpinConnection[-a, -b, i]])/3 - 2 * kR1 * CD[-a][SpinConnection[-l, a, -j]] * CD[l][SpinConnection[j, k, -k]] + 2 * kR1 * CD[-j][SpinConnection[-l, a, -a]] * CD[l][SpinConnection[j, k, -k]], TheoryName -> StringJoin["Case", ToString[51]], Method -> "Easy", MaxLaurentDepth -> 3];

==> LstListing/Line94.tex <==
In[94]:= ParticleSpectrum[-(kT1 * SpinConnection[-i, a, i] * SpinConnection[-k, -a, k]) - kT1 * SpinConnection[-i, k, l] * SpinConnection[-k, -l, i] - kR5 * CD[-i][SpinConnection[k, l, -k]] * CD[i][SpinConnection[-l, a, -a]] - (2 * kR1 * CD[b][SpinConnection[j, a, -k]] * CD[-j][SpinConnection[-a, -b, (*omitted 1824 characters for brevity*) l, a]] * CD[-l][SpinConnection[-a, -b, i]])/3 + kR5 * CD[-a][SpinConnection[-l, a, -j]] * CD[l][SpinConnection[j, k, -k]] - kR5 * CD[-j][SpinConnection[-l, a, -a]] * CD[l][SpinConnection[j, k, -k]], TheoryName -> StringJoin["Case", ToString[52]], Method -> "Easy", MaxLaurentDepth -> 3];

==> LstListing/Line95.tex <==
In[95]:= ParticleSpectrum[-(kT1 * SpinConnection[-i, a, i] * SpinConnection[-k, -a, k]) - kT1 * SpinConnection[-i, k, l] * SpinConnection[-k, -l, i] + kR1 * CD[-i][SpinConnection[k, l, -k]] * CD[i][SpinConnection[-l, a, -a]] - (2 * kR1 * CD[b][SpinConnection[j, a, -k]] * CD[-j][SpinConnection[-a, -b, (*omitted 1824 characters for brevity*) l, a]] * CD[-l][SpinConnection[-a, -b, i]])/3 - kR1 * CD[-a][SpinConnection[-l, a, -j]] * CD[l][SpinConnection[j, k, -k]] + kR1 * CD[-j][SpinConnection[-l, a, -a]] * CD[l][SpinConnection[j, k, -k]], TheoryName -> StringJoin["Case", ToString[53]], Method -> "Easy", MaxLaurentDepth -> 3];

==> LstListing/Line96.tex <==
In[96]:= ParticleSpectrum[-(kT1 * SpinConnection[-i, a, i] * SpinConnection[-k, -a, k]) - kT1 * SpinConnection[-i, k, l] * SpinConnection[-k, -l, i] + 2 * kR1 * CD[-i][SpinConnection[k, l, -k]] * CD[i][SpinConnection[-l, a, -a]] - (2 * kR1 * CD[b][SpinConnection[j, a, -k]] * CD[-j][SpinConnection[-a, -b, (*omitted 1848 characters for brevity*) l, a]] * CD[-l][SpinConnection[-a, -b, i]])/3 - 2 * kR1 * CD[-a][SpinConnection[-l, a, -j]] * CD[l][SpinConnection[j, k, -k]] + 2 * kR1 * CD[-j][SpinConnection[-l, a, -a]] * CD[l][SpinConnection[j, k, -k]], TheoryName -> StringJoin["Case", ToString[54]], Method -> "Easy", MaxLaurentDepth -> 3];

==> LstListing/Line97.tex <==
In[97]:= ParticleSpectrum[-1/3 * (kT1 * SpinConnection[-i, a, i] * SpinConnection[-k, -a, k]) - kT1 * SpinConnection[-i, k, l] * SpinConnection[-k, -l, i] + kR1 * CD[-i][SpinConnection[k, l, -k]] * CD[i][SpinConnection[-l, a, -a]] - (2 * kR1 * CD[b][SpinConnection[j, a, -k]] * CD[-j][SpinConnection[-a, -b, (*omitted 1858 characters for brevity*) l, a]] * CD[-l][SpinConnection[-a, -b, i]])/3 - kR1 * CD[-a][SpinConnection[-l, a, -j]] * CD[l][SpinConnection[j, k, -k]] + kR1 * CD[-j][SpinConnection[-l, a, -a]] * CD[l][SpinConnection[j, k, -k]], TheoryName -> StringJoin["Case", ToString[55]], Method -> "Easy", MaxLaurentDepth -> 3];

==> LstListing/Line98.tex <==
In[98]:= ParticleSpectrum[-(kT1 * SpinConnection[-i, a, i] * SpinConnection[-k, -a, k]) - (kT1 * SpinConnection[-i, k, l] * SpinConnection[-k, -l, i])/3 + (kT1 * SpinConnection[-k, -l, i] * SpinConnection[k, l, -i])/3 + 2 * kR1 * CD[-i][SpinConnection[k, l, -k]] * CD[i][SpinConnection[-l, a, -a]] - (2 * (*omitted 2152 characters for brevity*) l, a]] * CD[-l][SpinConnection[-a, -b, i]])/3 - 2 * kR1 * CD[-a][SpinConnection[-l, a, -j]] * CD[l][SpinConnection[j, k, -k]] + 2 * kR1 * CD[-j][SpinConnection[-l, a, -a]] * CD[l][SpinConnection[j, k, -k]], TheoryName -> StringJoin["Case", ToString[56]], Method -> "Easy", MaxLaurentDepth -> 3];

==> LstListing/Line99.tex <==
In[99]:= ParticleSpectrum[-(kT1 * SpinConnection[-i, a, i] * SpinConnection[-k, -a, k]) - (kT1 * SpinConnection[-i, k, l] * SpinConnection[-k, -l, i])/3 + (kT1 * SpinConnection[-k, -l, i] * SpinConnection[k, l, -i])/3 + 2 * kR1 * CD[-i][SpinConnection[k, l, -k]] * CD[i][SpinConnection[-l, a, -a]] - (2 * (*omitted 2732 characters for brevity*) l, a]] * CD[-l][SpinConnection[-a, -b, i]])/3 - 2 * kR1 * CD[-a][SpinConnection[-l, a, -j]] * CD[l][SpinConnection[j, k, -k]] + 2 * kR1 * CD[-j][SpinConnection[-l, a, -a]] * CD[l][SpinConnection[j, k, -k]], TheoryName -> StringJoin["Case", ToString[57]], Method -> "Easy", MaxLaurentDepth -> 3];
